CodeCloak: A Method for Evaluating and Mitigating Code Leakage by LLM Code Assistants

LLM-based code assistants are becoming increasingly popular among developers. These tools help developers improve their coding efficiency and reduce errors by providing real-time suggestions based on the developer's codebase. While beneficial, the use of these tools can inadvertently expose the developer's proprietary code to the code assistant service provider during the development process. In this work, we propose a method to mitigate the risk of code leakage when using LLM-based code assistants. CodeCloak is a novel deep reinforcement learning agent that manipulates the prompts before sending them to the code assistant service. CodeCloak aims to achieve the following two contradictory goals: (i) minimizing code leakage, while (ii) preserving relevant and useful suggestions for the developer. Our evaluation, employing StarCoder and Code Llama, LLM-based code assistants models, demonstrates CodeCloak's effectiveness on a diverse set of code repositories of varying sizes, as well as its transferability across different models. We also designed a method for reconstructing the developer's original codebase from code segments sent to the code assistant service (i.e., prompts) during the development process, to thoroughly analyze code leakage risks and evaluate the effectiveness of CodeCloak under practical development scenarios.

==> sec/3_background.tex <==
\section{\label{sec:drl}Deep Reinforcement Learning}
Reinforcement learning (RL) is an area of machine learning (ML) that addresses multi-step decision-making processes.
An RL algorithm normally consists of an agent that interacts with an environment in a sequence of actions and rewards.
In each time step $t$, the agent selects an action $a_i \in A$ = $\{a_{1}, a_{2}, ..., a_{k}\}$.
As a result of $a_i$, the agent transitions from the current state $s_t$ to a new state $s_{t+1}$. 
The selection of the action may result in a reward, which can be either positive or negative. 
The goal of the agent in each state is to interact with the environment in a way that maximizes the sum of future rewards $G_{t}$.
Eq.~\ref{eq:reward} represents the cumulative reward over time:
\begin{equation}
\label{eq:reward}
G_t = \sum_{k=0}^{\infty} \gamma^k R_{t+k+1}
\end{equation}
where:
\begin{itemize}
    \item $G_t$ is the expected return at step $t$.
    \item $R_{t+k+1}$ represents the reward received after $k$ steps from step $t$.
    \item $\gamma \in [0,1]$ is the discount factor, which provides the present value to future rewards. 
    A reward received $k$ steps in the future is valued at $\gamma^k$ times its immediate value.
\end{itemize}

In order to maximize Eq.~\ref{eq:reward}, the agent needs to learn its optimal policy. 
The policy defines how the agent behaves at any given time; i.e., which action to select when in a given state.
When faced with complex environments with high-dimensional data, it is common to use DRL, i.e., incorporate deep neural networks to learn the optimal policy.
This enables the agent to learn more sophisticated strategies and make more informed decisions. 
DRL algorithms can efficiently explore vast state and action spaces and devise strategies for addressing complex problems. 
Moreover, DRL excels in handling partial and noisy information. 
Utilizing the reward function, DRL algorithms can reconcile multiple, sometimes conflicting objectives, making them invaluable in security-related scenarios.



==> sec/table_actions.tex <==
\begin{table}[!ht] 
\centering
\captionsetup{justification=centering,singlelinecheck=false}
\caption{Code manipulation actions} 
\scalebox{0.5}{
\begin{tabular}{ll}
\toprule
\textbf{Action} & \textbf{Description} \\
\midrule
Change Variable Names & {Replace all variable identifiers in the current code segment with random strings of a fixed length (5 characters) consisting of letters and numbers.} \\
\midrule
Change Argument Names & Replace all argument identifiers in the current code segment with random strings of a fixed length (5 characters) consisting of letters and numbers. \\
\midrule
Change Function Names & Replace all function identifiers in the current code segment with random strings of a fixed length (5 characters) consisting of letters and numbers. \\
\midrule
Change Random Lines & Swap positions of two random lines present in the current code segment. \\
\midrule
Delete Random Line & Remove a random line from the current code segment. \\
\midrule
Insert Random Line & Insert a random line in the current code segment. \\
\midrule
Delete Function Bodies & Remove all function bodies present in the current code segment and replace them with summarization comments describing the original function bodies. \\
\midrule
Delete Function Bodies (Keep Last) & Remove all function bodies except the last one in the current code segment and replace the removed bodies with summarization comments (that were generated using a local summarization model). \\
\midrule
Delete Functions Incrementally & Incrementally remove functions from the current code segment. \\
\midrule
Delete Functions body Incrementally & Incrementally remove function bodies from the current code segment and replace the removed body replaced with summarization comments (that were generated using a local summarization model).\\
\midrule
Detect and Replace PII & Detect PII (e.g., names, API keys, emails) in the current code segment and replace them with random strings of a fixed length. \\
\midrule
Stop Manipulations & Stop processing the current prompt and send it to the code assistant service without further manipulations. \\
\bottomrule
\end{tabular}
}
%\vspace{0.5mm} % Adjust the space as needed
%\caption{Code manipulation actions} % Adjusted caption style as per your request
\label{tab:actions}
\end{table}

